Variational Federated Multi-Task Learning

In federated learning, a central server coordinates the training of a single model on a massively distributed network of devices. This setting can be naturally extended to a multi-task learning framework, to handle real-world federated datasets that typically show strong statistical heterogeneity among devices. Despite federated multi-task learning being shown to be an effective paradigm for real-world datasets, it has been applied only on convex models. In this work, we introduce VIRTUAL, an algorithm for federated multi-task learning for general non-convex models. In VIRTUAL the federated network of the server and the clients is treated as a star-shaped Bayesian network, and learning is performed on the network using approximated variational inference. We show that this method is effective on real-world federated datasets, outperforming the current state-of-the-art for federated learning, and concurrently allowing sparser gradient updates.

==> figures/lateral_connection.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tikzpicture}[
node distance=1cm and 0.5cm,
mynode/.style={
  draw,
  text width=6cm,
  align=center,
  text height=3ex,
  text depth=1.5ex,
}
]
\node[mynode, text width=2cm] (y) {Label};
\node[mynode, text width=4cm,below=of y]  (c1) {$h^c_3$};
\node[mynode, text width=4cm,below=2cm of c1] (c2) {$h^c_2$};
\node[mynode, text width=4cm,below=2cm of c2] (c3) {$h^c_1$};
\node[mynode, below right=1cm and -2cm of c3] (x) {Input};
\node[latent, below=0.6cm of c2]          (add3) {+};
\node[latent, right=2cm of add3]          (gate3) {Gate};
\node[mynode, text width=4cm,right=3cm of c2]  (s2) {$h^s_2$};
\node[latent, below=0.6cm of c1]          (add2) {+};
\node[latent, right=2cm of add2]          (gate2) {Gate};
\node[mynode, text width=4cm,right=3cm of c3]  (s3) {$h^s_1$};

\edge {x}{c3};
\edge {c3}{add3};
\edge {add3}{c2};
\edge {c2}{add2};
\edge {add2}{c1};
\edge {c1}{y};

\edge {x}{s3};
\edge {s3}{s2};

\tikzstyle{l} = [draw, -latex',thick]

\path [l] (s3) |- (gate3);
\edge {gate3}{add3};
\edge {add3}{c2};
\path [l] (s2) |- (gate2);
\edge {gate2}{add2};
\edge {add2}{c1};
{\tikzset{plate caption/.append style={below=3pt of #1.south west}}
\plate[dashed, inner sep=0.3cm] {Client} {(c1)(c2)(c3)(gate2)(gate3)} {Client parameters};}
\plate[dashed, inner sep=0.3cm] {Server} {(s2)(s3)}{Server parameters} ;
\end{tikzpicture}}
\caption{Depiction of the a Server-Client multi-layer perceptron model with two hidden layers and lateral connections. The server parameters on the right plate are shared between all the clients, while the client parameters on the left plate are private. See text for full details.}
\label{fig:lateral_connection}
